Efficient and effective training of language and graph neural network models

Can we combine heterogenous graph structure with text to learn high-quality semantic and behavioural representations? Graph neural networks (GNN)s encode numerical node attributes and graph structure to achieve impressive performance in a variety of supervised learning tasks. Current GNN approaches are challenged by textual features, which typically need to be encoded to a numerical vector before provided to the GNN that may incur some information loss. In this paper, we put forth an efficient and effective framework termed language model GNN (LM-GNN) to jointly train large-scale language models and graph neural networks. The effectiveness in our framework is achieved by applying stage-wise fine-tuning of the BERT model first with heterogenous graph information and then with a GNN model. Several system and design optimizations are proposed to enable scalable and efficient training. LM-GNN accommodates node and edge classification as well as link prediction tasks. We evaluate the LM-GNN framework in different datasets performance and showcase the effectiveness of the proposed approach. LM-GNN provides competitive results in an Amazon query-purchase-product application.

==> draft_tables.tex <==

\begin{table*}[t!]
\caption{Edge classification results for the public ESCI dataset. The performance is measured in F1-score, all classes reported. 
}
\vspace{0.1cm}
\centering
\setlength{\tabcolsep}{2.5pt}
\label{tab:arxiv}
%\scriptsize
\begin{tabular}{llllccccc}
\toprule
%\multicolumn{1}{l}{} 
 Semantic encoder& Graph encoder & Warm-start & Fine-tune &
  {EvSvCvI} & E & S & C & I \\ \midrule
  \rownumber~~ BERT-M5&MLP & No &No &
  {32.62} & 57.42& 38.12& 14.21 & 20.56 \\
\rownumber~~ BERT-M5&MLP & No &Yes &
  {37.36} & 59.25& 36.13& 21.23& 32.34\\ 
\rownumber~~ BERT-M5-GNN&MLP & No &No &
  {38.02}  & 57.34& 37.72& 22.63& 34.56\\
\rownumber~~ BERT-M5-GNN&MLP & No &Yes &
  {37.98}  & 55.71& 37.53& 21.85& 32.82\\ 
\rownumber~~  BERT-M5&GNN &No &No &
  {35.12} & 53.34& 38.21& 25.23& 25.42\\
 \rownumber~~  BERT-M5&GNN &No &Yes &
  \textbf{40.56} & \textbf{61.90}& 42.21& {26.30}& {30.21}  \\ 
 \rownumber~~  BERT-M5&GNN &Yes &Yes &
  {40.23} & 60.21& \textbf{45.21}& 30.02& 30.11\\ 
  %make the names better since we also use graph sage.
\rownumber~~ BERT-EP&GNN &No &No&
  {37.43} & 55.62&   43.22&  \textbf {32.60}& \textbf {35.24}\\ 
\rownumber~~  BERT-EP&GNN &No &Yes&
  {39.51}  & 60.81& 42.45& 21.56& 28.80\\ 
  \rownumber~~  BERT-EP&GNN &Yes &Yes&
 {40.13} & 60.90& 43.82& 18.20& {31.52}\\ 
  \bottomrule
  \vspace{-2em}
\end{tabular}
\vspace{-0.2cm}
\end{table*}


\begin{table*}[t!]
\caption{Edge classification results for the private ESCI dataset. The performance is measured in accuracy.
}
\vspace{0.1cm}
\centering
\setlength{\tabcolsep}{2.5pt}
\label{tab:arxiv}
%\scriptsize
\begin{tabular}{llllcH}
\toprule
%\multicolumn{1}{l}{} 
 Encoder& Decoder & Warm-start & Fine-tune &
  {E v SCI} \\ \midrule
  \rownumber~~ BERT-M5&MLP & No &No &
  {76.85} &
  {82.29}   \\
\rownumber~~ BERT-M5&MLP & No &Yes &
  { 88.19} &
  {82.29}   \\ 
\rownumber~~ BERT-M5-GNN&MLP & No &No &
  {83.65} &
  {82.29}   \\
\rownumber~~ BERT-M5-GNN&MLP & No &Yes &
  { 88.21} &
  {82.29}   \\ 
\rownumber~~  BERT-M5&GNN &No &No &
  {83.21} &
  83.53\\ 
 \rownumber~~  BERT-M5&GNN &No &Yes &
  {85.73} &
  83.53\\ 
 \rownumber~~  BERT-M5&GNN &Yes &Yes &
  {86.12} &
  83.53\\ 
  %make the names better since we also use graph sage.
\rownumber~~ BERT-EP&GNN &No &No&
  {88.21} &
  {81.34} \\ 
\rownumber~~  BERT-EP&GNN &No &Yes&
  {88.51} &
  {83.63} \\ 
  \rownumber~~  BERT-EP&GNN &Yes &Yes&
 \textbf{88.58} &
  \textbf{87.23} \\ 
  \bottomrule
  \vspace{-2em}
\end{tabular}
\vspace{-0.2cm}
\end{table*}


\begin{table*}[t!]
\caption{Edge classification results for the public ESCI dataset. The performance is measured in F1-score. %Mean accuracy ($\%$) $\pm$ one standard deviation. Boldfaced numbers indicate the best performances of downstream models, while underlined numbers indicate the best performance of models with a standard GNN pipeline for downstream models using $\mathbf{X}_{\text{plain}}$ and $\mathbf{X}_{\text{SSLGNN}}$. Methods under $\mathbf{X}_{\text{GIANT}}$ (GIANT framework) are part of the ablation study.
}
\vspace{0.1cm}
\centering
\setlength{\tabcolsep}{2.5pt}
\label{tab:arxiv}
%\scriptsize
\begin{tabular}{llllc}
\toprule
%\multicolumn{1}{l}{} 
 Encoder& Decoder & Warm-start & Fine-tune &
  {E v S v C v I} \\ \midrule
  \rownumber~~ BERT-M5&MLP & No &No &
  {32.62} \\
\rownumber~~ BERT-M5&MLP & No &Yes &
  {37.36}  \\ 
\rownumber~~ BERT-M5-GNN&MLP & No &No &
  {38.02}   \\
\rownumber~~ BERT-M5-GNN&MLP & No &Yes &
  {37.98}   \\ 
\rownumber~~  BERT-M5&GNN &No &No &
  {35.12} \\
 \rownumber~~  BERT-M5&GNN &No &Yes &
  \textbf{40.56}  \\ 
 \rownumber~~  BERT-M5&GNN &Yes &Yes &
  {40.23} \\ 
  %make the names better since we also use graph sage.
\rownumber~~ BERT-EP&GNN &No &No&
  {37.43}  \\ 
\rownumber~~  BERT-EP&GNN &No &Yes&
  {39.51}  \\ 
  \rownumber~~  BERT-EP&GNN &Yes &Yes&
 {40.13} \\ 
  \bottomrule
  \vspace{-2em}
\end{tabular}
\vspace{-0.2cm}
\end{table*}



\begin{table*}[t!]
\caption{Node classification results for the public datasets. Results measured in accuracy. %Mean accuracy ($\%$) $\pm$ one standard deviation. Boldfaced numbers indicate the best performances of downstream models, while underlined numbers indicate the best performance of models with a standard GNN pipeline for downstream models using $\mathbf{X}_{\text{plain}}$ and $\mathbf{X}_{\text{SSLGNN}}$. Methods under $\mathbf{X}_{\text{GIANT}}$ (GIANT framework) are part of the ablation study.
}
\vspace{0.1cm}
\centering
\setlength{\tabcolsep}{2.5pt}
\label{tab:arxiv}
%\scriptsize
\begin{tabular}{llllccHc}
\toprule
%\multicolumn{1}{l}{} 
 Encoder& Decoder & Warm-start & Fine-tune &
  {arxiv} &
  {products} & {yelp-2layer} & {yelp-1layer}\\ \midrule
\rownumber~~ BERT&MLP & No &No &
  { 62.91} &
  {61.83}  & - & -\\ 
 \rownumber~~ BERT&MLP &No & Yes &
  { 72.98} &
  { 77.64} & - & - \\ 
 \rownumber~~ BERT-GNN&MLP & No &No &
  {73.61} &
  {-}  & - & -\\ 
   \rownumber~~ BERT-GNN&MLP & No &Yes &
  {74.17} &
  {-}  & - & -\\ 
 \rownumber~~ BERT&MLP & No &No &
  { 62.91} &
  {61.83}  & - & -\\ 
\rownumber~~  BERT&GNN &No &No &
  {71.39 } &
  79.10 & 61.13 & 65.81 \\ 
\rownumber~~ BERT&GNN &No &Yes &
  {73.42} &
  {81.24} & 66.36 & 73.06 \\ 
\rownumber~~ BERT&GNN &Yes &Yes &
   {74.33}& {81.41}
   & 69.35 & 73.82 \\
\rownumber~~ BERT-NP&GNN &No &No &
  { 75.16} &
  { 82.03} & - & - \\ 
\rownumber~~ BERT-NP&GNN &No &Yes &
  {75.12} &
  {81.84} & - & - \\ 
\rownumber~~ BERT-NP&GNN &Yes &Yes &
  \textbf{75.63} &
  \textbf{82.86} & - & - \\ 
  %make the names better since we also use graph sage.
\rownumber~~ BERT-LP&GNN &No &No&
  {73.79} &
  {80.53} & 67.51 & 66.88 \\ 
\rownumber~~  BERT-LP&GNN &No &Yes&
  {74.97} &
  {82.35} & 60.92 & \textbf{76.47}\\ 
\rownumber~~ GIANT-XRT&MLP& No &No &
  {73.08} &
  79.82 & - & -\\
\rownumber~~   GIANT-XRT&GNN& No &No &
  {74.59} &
  - & - & -\\
  \bottomrule
  \vspace{-2em}
\end{tabular}
\vspace{-0.2cm}
\end{table*}


\begin{comment}
\begin{table*}[t!]
\caption{Results for the arxiv and products datasets. Mean accuracy ($\%$) $\pm$ one standard deviation. Boldfaced numbers indicate the best performances of downstream models, while underlined numbers indicate the best performance of models with a standard GNN pipeline for downstream models using $\mathbf{X}_{\text{plain}}$ and $\mathbf{X}_{\text{SSLGNN}}$. Methods under $\mathbf{X}_{\text{GIANT}}$ (GIANT framework) are part of the ablation study.}
\vspace{0.1cm}
\centering
\setlength{\tabcolsep}{2.5pt}
\label{tab:arxiv}
%\scriptsize
\begin{tabular}{@{}cccccc|ccc@{}}
\toprule
\multicolumn{1}{l}{} &
  Dataset &
  \multicolumn{4}{c|}{arxiv} &
  \multicolumn{3}{c}{products} \\ \midrule
\multicolumn{1}{l}{} &
   &
  MLP &
  GraphSAGE &
  RevGAT &
  RevGAT+SelfKD &
  MLP &
  GraphSAINT &
  SAGN+SLE \\ \midrule
\multirow{2}{*}{$\mathbf{X}_{\text{plain}}$} &
  OGB-feat$^\dagger$ &
  55.50 ± 0.23 &
  { 71.49 ± 0.27 } &
  { 74.02 ± 0.18} &
  { 74.26 ± 0.17} &
  { 61.06 ± 0.08} &
  79.08 ± 0.24 &
  { 84.28 ± 0.14} \\
 &
  BERT$^\star$ &
  { 62.91 ± 0.60} &
  70.97 ± 0.33 &
  73.59 ± 0.10 &
  73.55 ± 0.41 &
  60.90 ± 1.09 &
  { 79.55 ± 0.85} &
  83.11 ± 0.18 \\ \midrule
\multirow{8}{*}{$\mathbf{X}_{\text{SSLGNN}}$} &
  OGB-feat+GZ &
  { 70.95 ± 0.38} &
  71.41 ± 0.09 &
  72.42 ± 0.16 &
  72.50 ± 0.08 &
  74.19 ± 0.55 &
  78.38 ± 0.21 &
  79.78 ± 0.11 \\
 &
  BERT$^\star$+GZ &
  70.46 ± 0.21 &
  71.24 ± 0.19 &
  72.33 ± 0.06 &
  72.30 ± 0.20 &
  OOM &
  OOM &
  OOM \\
 &
  OGB-feat+DGI &
  56.02 ± 0.16 &
  71.72 ± 0.26 &
  73.48 ± 0.14 &
  73.90 ± 0.26 &
  70.54 ± 0.13 &
  79.26 ± 0.16 &
  81.59 ± 0.14 \\
 &
  BERT$^\star$+DGI &
  59.42 ± 0.38 &
  72.15 ± 0.06 &
  73.24 ± 0.25 &
  73.60 ± 0.21 &
  73.62 ± 0.23 &
  81.29 ± 0.41 &
  82.90 ± 0.21 \\
 &
  OGB-feat+GAE &
  56.47 ± 0.08 &
  72.00 ± 0.27 &
  73.70 ± 0.28 &
  74.06 ± 0.10 &
  74.81 ± 0.22 &
  78.23 ± 0.10 &
  82.85 ± 0.11 \\
 &
  BERT$^\star$+GAE &
  62.11 ± 0.32 &
  72.72 ± 0.17 &
  { 74.26 ± 0.20} &
  { 74.48 ± 0.15} &
  78.42 ± 0.14 &
  82.74 ± 0.16 &
  { 84.42 ± 0.04} \\
 &
  OGB-feat+VGAE &
  56.70 ± 0.20 &
  72.04 ± 0.29 &
  73.59 ± 0.17 &
  73.95 ± 0.09 &
  74.66 ± 0.10 &
  78.65 ± 0.20 &
  83.06 ± 0.06 \\
 &
  BERT$^\star$+VGAE &
  62.48 ± 0.14 &
  { 72.92 ± 0.02} &
  74.21 ± 0.01 &
  74.44 ± 0.09 &
  { 78.81 ± 0.25} &
  { 82.80 ± 0.11} &
  84.40 ± 0.09 \\ \midrule
\multicolumn{1}{l}{\multirow{5}{*}{$\mathbf{X}_{\text{GIANT}}$}} &
  BERT+LP &
  67.33 ± 0.54 &
  66.61 ± 2.86 &
  75.50 ± 0.11 &
  75.75 ± 0.04 &
  73.83 ± 0.06 &
  81.66 ± 0.08 &
  82.33 ± 0.16 \\ \cmidrule(l){2-9} 
\multicolumn{1}{l}{} &
  NO TFIDF+ NO PIFA &
  69.33 ± 0.19 &
  73.41 ± 0.34 &
  74.95 ± 0.07 &
  75.16 ± 0.06 &
  74.16 ± 0.22 &
  80.70 ± 0.51 &
  81.63 ± 0.28 \\
\multicolumn{1}{l}{} &
  NO TFIDF+PIFA &
  72.74 ± 0.17 &
  74.43 ± 0.20 &
  75.88 ± 0.05 &
  76.06 ± 0.02 &
  78.91 ± 0.28 &
  81.54 ± 0.14 &
  82.22 ± 0.15 \\
\multicolumn{1}{l}{} &
  TFIDF+NO PIFA &
  71.74 ± 0.15 &
  74.09 ± 0.33 &
  75.56 ± 0.09 &
  75.85 ± 0.05 &
  79.37 ± 0.15 &
  83.83 ± 0.14 &
  85.01 ± 0.10 \\
\multicolumn{1}{l}{} &
  GIANT-XRT &
  \textbf{73.08 ± 0.06} &
  \textbf{74.59 ± 0.28} &
  \textbf{75.96 ± 0.09} &
  \textbf{76.12 ± 0.16} &
  \textbf{79.82 ± 0.07} &
  \textbf{84.40 ± 0.17} &
  \textbf{85.47 ± 0.29} \\
  \bottomrule
  \vspace{-2em}
\end{tabular}
\vspace{-0.2cm}
\end{table*}
\end{comment}

